Incorporating Gaze into Social Navigation

Most current approaches to social navigation focus on the trajectory and position of participants in the interaction. Our current work on the topic focuses on integrating gaze into social navigation, both to cue nearby pedestrians as to the intended trajectory of the robot and to enable the robot to read the intentions of nearby pedestrians. This paper documents a series of experiments in our laboratory investigating the role of gaze in social navigation.

==> figures/gaze_ahead_left.tex <==
\begin{figure}
    \vspace*{2mm}
    \centering
    \includegraphics[width=4cm]{figures/face_neutral.jpg}
    \includegraphics[width=4cm]{figures/face_signal.jpg}
    \caption{\jh{CHANGE Gaze Signal. Left: Neutral; Right: Signaling to the left lane.}}
    \label{fig:conditions_gaze_1}
\end{figure}

==> figures/passive_demonstrations_study_conditions.tex <==
\begin{table}[]
\centering
\begin{tabular}{llccll}
\cline{1-4}
\multicolumn{4}{|c|}{\textbf{Study Conditions}}                                                                                                                                                                      & &  \\ \cline{1-4}
\multicolumn{1}{|l}{} & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{Passive Demonstration}}                                                                                                                                &  &  \\ \cline{3-4}
\multicolumn{1}{|l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\textbf{No Demonstration}} & \multicolumn{1}{c|}{\textbf{Demonstration}} &  &  \\ \cline{1-4}
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}LED \\ Signal\end{tabular}}}} & \multicolumn{1}{c|}{\textbf{No LED}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}No Demonstration,\\ No LED\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Demonstration,\\ No LED\end{tabular}} &  &  \\ \cline{2-4}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\textbf{LED}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}No Demonstration,\\ LED\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Demonstration,\\ LED\end{tabular}} &  &  \\ \cline{1-4}
 & & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & 
\end{tabular}
\caption{Study Conditions}
\label{conditions}
\end{table}

==> figures/passive_demonstrations_turn_signal.tex <==
\begin{figure}
  \centering
  \begin{subfigure}{0.37\columnwidth}
  \centering
  	\includegraphics[width=0.9\columnwidth]{figures/leftturn}
  	\caption{Left turn signal.}	
  \end{subfigure}%
  \begin{subfigure}{0.37\columnwidth}
	\centering
  	\includegraphics[width=0.9\columnwidth]{figures/rightturn}
  	\caption{Right turn signal.}	
  \end{subfigure}
  	\caption{\jh{CHANGE CAPTIONS: Signal Animations for Directionality Intention.}}
  \label{fig:turn}
\end{figure}

==> figures/traffic_lanes_diagram.tex <==
\begin{figure}[t!]
  	\centering
  	\includegraphics[width=0.45\textwidth]{figures/diagram5.jpg}
  	\caption {\jh{CHANGE THIS TEXT. A diagram of the corridor, its lanes, and the distance thresholds at which the robot signals its intention to change lanes, executes a lane change, and is determined to potentially be in conflict with a person in its path. The position of the robot is marked $p_r$. The respective action for each distance is executed as the position, $p_h$, of the person crosses these distance thresholds.}}
  	\label{fig:diagram}
\end{figure}

==> passive_demonstrations_results_table.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{|l|l|l|}
\hline
No Demo, No LED & No Demo, LED & $M=0.1, p>0.5$\\
No Demo, No LED & Demo, No LED & $M=0.3, p=0.07$\\
\textbf{* No Demo, No LED} & \textbf{Demo, LED} & $\bm{M=0.8, p<0.01}$\\
\hline
No Demo, LED & Demo, No LED & $M=0.2, p=0.22$\\
\textbf{* No Demo, LED} & \textbf{Demo, LED} & $\bm{M=0.7, p<0.01}$\\
\hline
\textbf{* Demo, No LED} & \textbf{Demo, LED} & $\bm{M=0.5, p<0.01}$\\
\hline
\end{tabular}
\caption{Pairwise Comparison with LSD Post-Hoc Test.}
\label{pclsd}
\end{table}

==> previous_experiments.tex <==
\section{Previous Experiments}
LED signals, virtual head signal, VR gaze prediction
\xuesu{I have been thinking about separating this section into two sections: 1. The Effect of Gaze in Social Navigation for Humans (our human field study and the VR study), and 2. Instantiating Robot Gaze for Social Navigation (LED and vitual head). Or do we want to keep all four in this section?} \rdm{I don't have a preference whether this should be a single section with subsections or several different sections. I really like the titles of the three projects so I added it to the introduction as well.}

In this section, we report two human studies which investigate the effect of incorporating gaze as a navigational cue in social contexts. We also present two different approaches to instantiate gaze on a physical robot to improve human robot interaction in the context of social navigation. 

\subsection{Gaze to Disambiguate Navigational Intentions}
We conduct a human ecological field study, which investigates the effect of violating expected human gaze patterns while navigating a shared space. In a $2 \times 3$ study, research confederates look in a direction that is congruent with the direction that they intend to walk; opposite to the direction in which they intend to walk; or look down at their cell phone providing no gaze cue. The opposite gaze condition violates the gaze expectations observed by the work of Patla et al. \cite{Patla1999} and Unhlelkar et al. \cite{unhelkar2015human}, in which head pose is predictive of trajectory. The no gaze condition simply eliminates the gaze stimulus. Along the other axis of this study, we vary whether the interaction happens while the hallway is relatively crowded or relatively uncrowded. We hypothesize that violating expected gaze cues, or simply not providing them, causes problems in interpreting the navigational intent of the confederate, and can lead to confusion or near-collisions.

\subsubsection{EXPERIMENTAL SETUP}

The William C. Powers, Jr. Student Activity Center (WCP) at UT Austin is a busy, public building hosting meeting rooms for student activities and a variety of restaurants in its food court. It has predictable busy times, centering around the schedule of class changes at the university. This study was performed in a hallway which becomes crowded during class changes (see Figure \ref{fig:SAC}).

\begin{figure}[ht]
    \centering
    %4, 5
    \includegraphics[width=4.4cm]{figures/SAC.jpg}
    \includegraphics[width=5.5cm, angle=90]{figures/SAC_floor}
    \caption{The hallway in which the human field experiment took place.}
    \label{fig:SAC}
\end{figure}

Prior to this study, two of the authors of this paper trained each other to proficiently look counter to the direction in which they walk, and acted as confederates who interacted with study participants. Both of the confederates who participated in this study are females. A third author acted as a passive observer of interactions between these confederates and other pedestrians walking through the hallway.

This experiment is organized as a $2\times3$ study, controlling whether the interaction occurs in a ``crowded'' or ``uncrowded'' hallway, and whether the confederate looks in the direction in which they intend to go (their gaze is ``congruent''), opposite to this direction (their gaze is ``incongruent''), or focuses unto a mobile phone (``no gaze" is available). %An example of a congruent and an incongruent gaze conditions can be seen in the companion video. 
Here, ``crowded'' is defined as a state in which it is difficult for two people to pass each other in the hallway without coming within $2$m of each other. It can be observed that the busiest walkways at times form ``lanes'' in which pedestrians walk directly in lines when traversing these spaces. This study was not performed under these conditions, as walking directly toward another pedestrian would require additionally breaking these lanes, introducing another variable into the study.

The passive observer annotated all interactions in which the confederate and a pedestrian walked directly toward each other. If the confederate and the pedestrian had problems walking around each other or nearly collided with each other, the interaction was annotated as a ``conflict.'' Conflicts are further divided into ``full'' conflicts, in which the two parties (gently) bumped into each other; ``partial,'' in which the confederate and pedestrian brushed against each other; or ``shift,'' in which the two parties shifted to the left or right to deconflict each other's paths after coming into conflict.

\subsubsection{RESULTS}
\label{hum:results}
A total of $220$ interactions were observed ($130$ female / $90$ male), with $112$ in crowded conditions and $108$ in uncrowded conditions. In the crowded condition, the confederate looked in the congruent direction in $31$ interactions, in the incongruent direction in $41$ interactions, and no gaze in $40$. In the uncrowded condition, the confederate looked in the congruent direction in $29$ interactions, in the incongruent direction in $44$ interactions, and no gaze in $35$. A one-way ANOVA found no significant main effect between the crowded and uncrowded conditions ($F_{1,218}=1.49, p=0.22$), or based on gaze direction assuming the confederate looked either left or right ($F_{1,143}=1.28, p=0.26$).\footnote{Excluding the no-gaze condition, as it is fundamentally different.}  
Whether the confederate goes to the pedestrian's right or left during the interaction has a significant main effect ($F_{1,218}=9.44, p=0.002$), and so does whether the gaze is congruent with the walking direction or non-existent ($F_{2,217} = 5.02, p=0.007$). Post-hoc tests of between-groups differences using the Bonferroni criteria show significant mean differences between the congruent group and the other groups (congruent versus incongruent: $md=0.221, p=0.017$, congruent versus no gaze: $md=0.191, p=0.033$), but no significant mean difference between the incongruent and no gaze conditions ($md=-0.030, p=1.00$).

Observing the conflicting trajectories between the congruent and incongruent conditions shows that %going opposite to the direction of motion is a significantly misleading cue, and that 
gaze direction is a strong implicit communicative cue of intended trajectory. The relatively small difference between the incongruent and no gaze conditions may indicate that other motion cues are available in the no gaze condition which are dominated by (incongruent) gaze, or simply that people are more cautious when they know that others are not looking for them. A full breakdown of conflicts based on the congruent condition versus the incongruent gaze condition and the no-gaze condition can be found in Table \ref{tab:human}.

\begin{table}[ht]
\centering
\begin{tabular}{|c||c|c|c|}
\hline
\textbf{Conflict Type} & \textbf{Congruent} & \textbf{Incongruent} & \textbf{No Gaze}\\ \hline
Partial       & 9 (15\%)  & 11 (13\%)  & 7 (9\%)\\ \hline
Quick Shift   & 6 (10\%)  & 27 (32\%) & 13 (17\%)\\ \hline
Full          & 0 (0\%)        & 3 (4\%) & 1 (1\%)  \\ \hline \hline
Any Conflict & 15 (25\%)        & 41 (48\%) & 21 (28\%) \\ \hline 
No Conflict   & 45 (75\%)  & 44 (52\%)  & 54 (72\%) \\ \hline \hline
Total          & 60 (100\%) & 85 (100\%)  & 75 (100\%) \\ \hline
\end{tabular}
\caption{Human Field Study Results}
%\caption{Ratio of participants divided by congruence of gaze and walking direction contrasted with the type of conflict.}
\label{tab:human}
\vspace{-10pt}
\end{table}

\subsection{Gaze as Indication of Navigational Intentions}
\xuesu{VR study here}

\subsection{Instantiating Robot Gaze for Social Navigation}
Motivated by the use of gaze as a naturalistic cue for implicitly communicating navigational intent, we engineered a system in which a robot uses a virtual agent head to communicate the direction it intends to steer toward: in order to deconflict its trajectory from that of a human navigating a shared space, the robot gazes in the direction that it intends to navigate toward. In these experiments, a human starts at one end of a hallway, and the robot starts at the other end. The human is instructed to traverse the hallway to the other end, and the robot also autonomously traverses it. As a proxy for measuring understanding of the cue, the number of times that the human and robot come into conflict with each other is measured for two conditions; one in which the robot uses a turn signal to indicate the side of the hallway that it intends to pass the person on, and one in which it uses a gaze cue to make this indication. This experiment is motivated by prior work \cite{fernandez2018passive} which introduced the concept of a ``passive demonstration'' in order to overcome the challenge of people not understanding the intention of the turn signal. The question asked here is, ``Will the gaze cue be more easily interpreted than the turn signal, thus eliminating the need for the passive demonstration?'' Both cues are presented without the passive demonstrations developed by Fernandez et al. \cite{fernandez2018passive}. 

% \footnote{The robot's motion is intended to be similar to a car changing lanes.}

\begin{figure}[ht]
    \vspace*{2mm}
    \centering
    %6
    \includegraphics[width=8cm]{figures/hallway_occupied_not}
    \caption{The hallway constructed for this experiment (left) and a snapshot of the experiment during execution (right).}
    \label{fig:hallway}
\end{figure}

\begin{figure}[ht]
    \centering
    %8
    \includegraphics[width=8cm]{figures/lanes_cropped.png}
    \caption{The robot's mental map of the hallway.}
    \label{fig:lanes}
\end{figure}

This study is set in a test hallway built from cubicle furniture (see Figure \ref{fig:hallway}). The hallway is $17.5$m long by $1.85$m wide. The system models the problem of traversing the hallway as one in which the hallway is divided into three lanes, similar to traffic lanes on a roadway, as illustrated in Figure \ref{fig:lanes}. If the human and the robot come within $1$m of each other as they cross each other's path, they are considered to be in conflict with each other. This distance is based on the $1$m safety buffer engineered into the robot's navigational software, which also causes the robot to stop. If the human and the robot both start in the middle lane, at opposing ends of the hallway, with the navigational goal of traversing to the opposing ends of the hallway, the signal is intended to indicate an intended lane chance on behalf of the robot, so that the human may interpret that signal, and shift into the opposing lane if necessary. 


\subsubsection{GAZE AS LED SIGNAL}
The LED cue is a re-implementation of the LED turn signals from \cite{fernandez2018passive}. Strips of LEDs $0.475$m long with $14$ LEDs line the 8020 extrusion on the chassis of the front of the BWIBot. They are controlled using an Arduino Uno microcontroller, and blink twice per second with $0.25$ seconds on and $0.25$ seconds off each time they blink. In the condition that the LEDs are used, the monitor is removed from the robot. The LED signals can be seen in Figure \ref{fig:conditions_LED}.

\begin{figure}[ht]
    %\vspace*{2mm}
    \centering
    \includegraphics[width=4cm]{figures/led_neutral_2.jpg}
    \includegraphics[width=4cm]{figures/led_signal_3.jpg}
    \caption{LED signals. Left: Neutral; Right: Blinking to signal a move to the left lane.}
    \label{fig:conditions_LED}
\end{figure}


\subsubsection{GAZE AS VIRTUAL HEAD}

To display gaze cues on the BWIBot we developed a 3D-rendered version of the Maki 3D-printable robot head.\footnote{\url{https://www.hello-robo.com/maki}} The decision to use this head is motivated by the ability to both render it as a virtual agent and, in future work, to 3D print and assemble a head. The virtual version of the head was developed by converting the 3D-printable STL files into Wavefront .obj files and importing them into the Unity game engine.\footnote{\url{https://unity.com/}} To control the head and its gestures, custom software was developed using ROSBridgeLib.\footnote{\url{https://github.com/MathiasCiarlo/ROSBridgeLib}} The head is displayed on a $21.5$ inch monitor mounted to the front of the robot. When signaling, the robot turns its head $16.5^{\circ}$ and remains in this pose. The eyes are not animated to move independently of the head. The head turn takes $1.5$ seconds. These timings and angles were hand-tuned and pilot tested on members of the laboratory. The gaze signal can be seen in Figure \ref{fig:conditions_gaze_1}.


\begin{figure}
    \vspace*{2mm}
    \centering
    \includegraphics[width=4cm]{figures/face_neutral.jpg}
    \includegraphics[width=4cm]{figures/face_signal.jpg}
    \caption{Gaze Signal. Left: Neutral; Right: Signaling to the left lane.}
    \label{fig:conditions_gaze_1}
\end{figure}


\subsubsection{EXPERIMENTAL SETUP}
\label{sec:exp}

To test the effectiveness of gaze in coordinating navigation through a shared space, we conducted a human-robot interaction study in the hallway test environment. After obtaining informed consent and, optionally, media release, participants are guided to one end of the hallway, where the robot is already set up at the opposite end. The participant is instructed to navigate to the opposing end of the hallway, and both the participant and the robot start in the ``middle lane,'' as per the model in Section \ref{sec:gaze_cue}. When the participant starts walking down the hallway, the robot is also started. The study presented here is designed using an inter-participant design, in which each participant sees exactly one of the two cues -- gaze or LED. Each participant traverses the hallway with the robot exactly once in order to avoid training effects. After completing the task of walking down the hallway, each participant responds to a brief post-interaction survey.

To ensure that the study results are reflective of the robot's motion signaling behavior, rather than the participants' motion out of the robot's path, the study is tuned to give the participant enough time to get out of the robot's way if the decision is based on reacting to its gaze or LED cue, but not enough time if the decision is based on watching the robot's motion. This tuning was performed on the experimenters prior to the experiment.

The problem is modeled using three distances which are used in this tuning: $d_{\mbox{\emph{signal}}}$, $d_{\mbox{\emph{execute}}}$ and $d_{\mbox{\emph{conflict}}}$. The distance $d_{\mbox{\emph{signal}}}$ ($4$m) is the distance at which the robot signals its intention to change lanes, which is based on the distance at which the robot can accurately detect a person in the hallway using a leg detector \cite{leigh2015person} and its on-board LiDAR sensor. The distance at which the robot will execute its turn, $d_{\mbox{\emph{execute}}}$ ($2.75$m), is hand-tuned to be at a range at which it is unlikely that the participant will have time to react to the robot's gaze or LED cue. This design is so that if the participant has not already started changing lanes by the time the robot begins its turn, it is highly likely that the person and robot will experience a conflict. Thus, this study tests interpretation of the cue, not reaction to the turn. The distance at which the robot determines that its motion is in conflict with that of the study participant is $d_{\mbox{\emph{conflict}}}$, which is set to $1$m. This design is based on the safety buffer used when the robot is autonomously operating in our building. For this study, the robot is tuned to move at a speed of $0.75$(m/s), which is the speed the robot moves when deployed in our building. Average human walking speed is about $1.4$(m/s).

In addition to using these three ranges to control the robot's behavior, the robot also always moves itself into the ``left'' lane. This choice was made because, in North America, pedestrians usually walk to the right of each other in order to deconflict each other's paths. This behavior is shown to be significant in our human field study as well, in Section \ref{hum:results}. Fernandez et al. conducted a  pilot study \cite{fernandez2018passive} to test how often humans and the robot come into conflict when the robot goes to the left lane, rather than into the right lane, with no cue, such as an LED or gaze cue. That study showed that the pedestrians and the robot came into conflict $100\%$ of the time under this regime. By choosing the behavior of the robot going into the left lane and beginning its turn at the last possible moment that would deconflict its trajectory from that of the person --- and such that the motion would be deconflicted only in the case that the person chooses to go into the opposite lane --- we can attribute cases in which the robot and the study participant successfully coordinate their trajectories primarily to the robot's signaling.

After the interaction, a post-interaction survey is administered. The survey comprises $44$ questions, consisting of $8$-point Likert and cognitive-differences scales, and one free-response question. Five demographic questions on the survey ask whether people in the country where the participant grew up drive or walk on the left or right-hand side of the road and about their familiarity with robots. The questions from the survey are available online.\footnote{\url{https://drive.google.com/drive/folders/1qVj-gU1aFwY6Eq2a_l9ZdesfmQ_QQOC8?usp=sharing} \\ The first question ``Condition'' was filled in before participants responded.}

%Ten questions concern factors such as the clarity of the signaling method used by the robot. Finally, twenty nine questions ask about perceptions of the robot in terms of personality factors such as selfishness or whether the robot is perceived as threatening; factors of safety and usefulness; and other factors such as appropriate environments for the robot, such as the workplace or home. The free response prompts the following to participants in the LED condition, ``There would be a better position for the signals, and it is:'' 

\subsubsection{RESULTS}
We recruited $38$ participants ($26$ male / $12$ female), ranging in age from $18$ to $33$ years. The data from $11$ participants is excluded from our analysis due to software failure or failure in participation of the experimental protocol. 

The remaining pool of participants includes $11$ participants in the LED condition and $16$ in the gaze condition. Table \ref{tab:robot} shows the results from the robot signaling experiment in these two conditions. A pre-test for homogeneity of variances confirms the validity of a one-way ANOVA for analysis of the collected data. A one-way ANOVA shows a significant main effect ($F_{1,35}=7.711$, $p=0.002$). Post-hoc tests of between-groups differences using the Bonferroni criteria show significant mean differences between the gaze group and the LED group (gaze versus LED: $md=-0.50, se=0.14, p=0.004$), but no significant mean difference between the gaze and LED conditions ($md=-0.08, se=0.15, p=1.00$). None of the post-interaction survey responses revealed significant results.\footnote{Example interactions can be seen in the companion video to this paper, posted at
\noindent \url{https://youtu.be/rQziUQro9BU}.} These results support the hypothesis that the robot's gaze can be more readily interpreted in order to deconflict its trajectory from that of a person navigating in a shared space.

%\xuesu{need to update the video, at least the title of the video to match with the new paper title}

\begin{table}[ht]
%\vspace*{2mm}
\centering
\begin{tabular}{|c||c|c|c|}
\hline
             \textbf{}  & \textbf{LED}         & \textbf{Gaze}           \\ \hline
\textbf{Conflict}       & 11 (100\%)         & 8 (50\%)                  \\ \hline
\textbf{No Conflict}    & 0 (0\%)          & 8 (50\%)                   \\ \hline \hline
Total & 11 & 16    \\ \hline
\end{tabular}
\caption{Experimental Results}
\label{tab:robot}
\vspace{-10pt}
\end{table}


\input{figures/traffic_lanes_diagram}
\input{figures/passive_demonstrations_study_conditions}
\input{figures/passive_demonstrations_turn_signal}
\input{passive_demonstrations_results_table}

\input{figures/gaze_ahead_left}


